The Shortest Route Is Not Always the Fastest: Probability-Modeled Stereoscopic Eye Movement Completion Time in VR

Speed and consistency of target-shifting play a crucial role in human ability to perform complex tasks. Shifting our gaze between objects of interest quickly and consistently requires changes both in depth and direction. Gaze changes in depth are driven by slow, inconsistent vergence movements which rotate the eyes in opposite directions, while changes in direction are driven by ballistic, consistent movements called saccades, which rotate the eyes in the same direction. In the natural world, most of our eye movements are a combination of both types. While scientific consensus on the nature of saccades exists, vergence and combined movements remain less understood and agreed upon. We eschew the lack of scientific consensus in favor of proposing an operationalized computational model which predicts the speed of any type of gaze movement during target-shifting in 3D. To this end, we conduct a psychophysical study in a stereo VR environment to collect more than 12,000 gaze movement trials, analyze the temporal distribution of the observed gaze movements, and fit a probabilistic model to the data. We perform a series of objective measurements and user studies to validate the model. The results demonstrate its predictive accuracy, generalization, as well as applications for optimizing visual performance by altering content placement. Lastly, we leverage the model to measure differences in human target-changing time relative to the natural world, as well as suggest scene-aware projection depth. By incorporating the complexities and randomness of human oculomotor control, we hope this research will support new behavior-aware metrics for VR/AR display design, interface layout, and gaze-contingent rendering.

==> Makefile <==
FINAL = out_final
DRAFT = out_draft

.PHONY: clean

all: final draft

final: $(FINAL).manuscript.compressed.pdf $(FINAL).supplement.compressed.pdf $(FINAL).all.compressed.pdf
draft: $(DRAFT).manuscript.compressed.pdf $(DRAFT).supplement.compressed.pdf $(DRAFT).all.compressed.pdf

%.compressed.pdf : %.pdf
	gs -sDEVICE=pdfwrite -dCompatibilityLevel=1.5 -dNOPAUSE -dQUIET -dBATCH -dPrinted=false -sOutputFile=$*.compressed.pdf $*.pdf

%.supplement.pdf : %.manuscript.pdf %.all.pdf
	gs -dNOPAUSE -dQUIET -dBATCH -sOutputFile="$*.supplement.pdf" -dFirstPage=$$(echo $$(gs -q -dNODISPLAY -dNOSAFER -c "($*.manuscript.pdf) (r) file runpdfbegin pdfpagecount = quit") + 1 | bc) -dLastPage=$$(gs -q -dNODISPLAY -dNOSAFER -c "($*.all.pdf) (r) file runpdfbegin pdfpagecount = quit") -sDEVICE=pdfwrite "$*.all.pdf"

%.manuscript.pdf : %.all.pdf
	# Make manuscript version of paper.tex
	cat $*.tex | sed 's/\\\input{paper}/\\\input{paper.manuscript}/' > $*.manuscript.tex
	# First generate support files
	cat paper.tex | sed 's/^.*\\\includeonly{}/% \\\includeonly{}/' > paper.manuscript.tex
	pdflatex -jobname=$*.manuscript $*.manuscript.tex
	# Remove supplement section
	cat paper.tex | sed 's/^.*\\\includeonly{}/\\\includeonly{}/' > paper.manuscript.tex
	pdflatex -jobname=$*.manuscript $*.manuscript.tex
	bibtex $*.manuscript.aux
	pdflatex -jobname=$*.manuscript $*.manuscript.tex
	pdflatex -jobname=$*.manuscript $*.manuscript.tex
	# Clean-up temporary files
	rm -f paper.manuscript.tex $*.manuscript.tex

%.all.pdf :
	pdflatex -jobname=$*.all $*.tex
	bibtex $*.all.aux
	pdflatex -jobname=$*.all $*.tex
	pdflatex -jobname=$*.all $*.tex

clean:
	rm -f *.blg *.aux *.log *.out *.cut
	rm -f *.all.bbl *.manuscript.bbl *.supplement.bbl
	rm -f *.all.compressed.pdf *.all.pdf
	rm -f *.all-support.tex
	rm -f *.manuscript.compressed.pdf *.manuscript.pdf
	rm -f *.manuscript-support.tex
	rm -f *.supplement.compressed.pdf *.supplement.pdf


==> fig_supp_ablation_histograms.tex <==
\begin{figure}[h]
    \centering
    \subfloat[$\conditionAccuracySaccade$, divergent]{
        \includegraphics[width=0.47\linewidth]{figures/pilot_data_histograms_divergent_saccade.pdf}
        \label{fig:supp:ablation:saccade:div}
    }%subfloat
    \subfloat[$\conditionAccuracySaccade$, convergent]{
        \includegraphics[width=0.47\linewidth]{figures/pilot_data_histograms_convergent_saccade.pdf}
        \label{fig:supp:ablation:saccade:con}
    }%subfloat
    
    \subfloat[$\conditionAccuracyVergence$, divergent]{
        \includegraphics[width=0.47\linewidth]{figures/pilot_data_histograms_divergent_vergence.pdf}
        \label{fig:supp:ablation:vergence:div}
    }%subfloat
    \subfloat[$\conditionAccuracyVergence$, convergent]{
        \includegraphics[width=0.47\linewidth]{figures/pilot_data_histograms_convergent_vergence.pdf}
        \label{fig:supp:ablation:vergence:con}
    }%subfloat
    
    \Caption{
        Histograms vs. predicted distributions of ablation models.
    }{
        Predicted distributions by the ablation models are compared to measured data from psychophysical study.
        Ablation model $\conditionAccuracySaccade$ was trained using only saccade amplitude information from the study data, while $\conditionAccuracyVergence$ only used vergence amplitude information.
        Since either model does not have full information that distinguishes individual conditions within a single column and row respectively, the models make the same predictions across multiple conditions within this histogram visualization.
        Thus, in \subref{fig:supp:ablation:saccade:div}/\subref{fig:supp:ablation:saccade:con} the model makes the same prediction within the same columns, while in \subref{fig:supp:ablation:vergence:div}/\subref{fig:supp:ablation:vergence:con} the model makes the same predictions within the same rows.
    }
\end{figure}

==> fig_supp_eval_tile.tex <==
\begin{figure}[h]
    \centering
    \begin{tabular}{ m{0.06\linewidth} m{0.04\linewidth} m{0.04\linewidth} c c c }
        user & D & p & archery & basketball & natural\\        
        \hline
        \\
        $U_1$ & 0.2 & 1.0 & 
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/0_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/0_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/0_2.pdf}
        \end{minipage}
        \\ 
        
        $U_2$ & 0.3 & .79 &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/1_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/1_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/1_2.pdf}
        \end{minipage}
        \\    
        
        $U_3$ & 0.2 & 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/2_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/2_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/2_2.pdf}
        \end{minipage}
        \\  
        
        $U_4$ & 0.1& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/3_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/3_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/3_2.pdf}
        \end{minipage}
        \\  
        
        $U_5$ &0.2& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/4_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/4_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/4_2.pdf}
        \end{minipage}
        \\  
        
        $U_6$ &0.1& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/5_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/5_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/5_2.pdf}
        \end{minipage}
        \\         
        
        $U_7$ &0.1& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/6_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/6_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/6_2.pdf}
        \end{minipage}
        \\  
        
        $U_8$ &0.2& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/7_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/7_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/7_2.pdf}
        \end{minipage}
        \\  
        
        $U_9$ &0.1& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/8_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/8_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/8_2.pdf}
        \end{minipage}
        \\  
        
        $U_{10}$ &0.2& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/9_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/9_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/9_2.pdf}
        \end{minipage}
        \\       
        
        $U_{11}$ &0.2& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/10_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/10_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/10_2.pdf}
        \end{minipage}
        \\          
        
        $U_{12}$ &0.2& 1.0&
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/11_0.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/11_1.pdf}
        \end{minipage}
        &
        \begin{minipage}{.095 \textwidth}
            \includegraphics[width=\linewidth]{figures/eval_tile_new/11_2.pdf}
        \end{minipage}
        \\          
    \end{tabular}
    \Caption{Visualization of all participants, conditions and scenes of the user study \Cref{sec:results:study}.
    }{%
    X-axis indicates time (0-1000ms). Y-axis indicates density. Each color of the stacked bars indicates each condition: blue/red/green represents $\conditionEvalStudyVergent:\vergentAmp= 0^\circ$ / $\conditionEvalStudyCombinedShort:\vergentAmp= 7^\circ$ / $\conditionEvalStudyCombinedLong:\vergentAmp= 10.5^\circ$. The inset numbers are the corresponding K.S. test results for each user across all conditions and scenes. Note that the  discrepancy between eye travel distance ($\conditionEvalStudyVergent<\conditionEvalStudyCombinedShort<\conditionEvalStudyCombinedLong$) and landing times ($\conditionEvalStudyCombinedShort<\conditionEvalStudyCombinedLong<\conditionEvalStudyVergent$) share statistical significance across individuals.
    }
    \label{fig:appendix:eval}
\end{figure}


==> fig_supp_results_errorbars.tex <==
\begin{figure}[h]
    \centering
    \subfloat[saccade]{
        \vphantom{\includegraphics[width=0.290\linewidth,valign=t]{figures/pilot_data_aggregate_divergent_errorbar.pdf}}
        \includegraphics[width=0.330\linewidth,valign=t]{figures/pilot_data_aggregate_saccade_errorbar.pdf} \label{fig:supp:results:saccade}
    }%subfloat
    \subfloat[divergent]{
        \includegraphics[width=0.290\linewidth,valign=t]{figures/pilot_data_aggregate_divergent_errorbar.pdf}
        \label{fig:supp:results:divergent}
    }%subfloat
    \subfloat[convergent]{
        \includegraphics[width=0.290\linewidth,valign=t]{figures/pilot_data_aggregate_convergent_errorbar.pdf}
        \label{fig:supp:results:convergent}
    }%subfloat
    \Caption{
        Aggregated mean offset time of studied conditions across all participants with error bars.
    }{%
        This is a version of \Cref{fig:pilot:summary} with std error bars as a more detailed visualization.
        See \Cref{fig:pilot:summary} for further details.
    }
\label{fig:supp:results}
\end{figure}


==> fig_supp_study_conditions.tex <==
\begin{figure}[h]
    \centering
    \subfloat[divergent]{
        \includegraphics[width=0.45\linewidth]{figures/angle-def/divergent-cond.pdf}
        \label{fig:supp:study:conditions:divergent}
    }%subfloat
    \hfill
    \subfloat[convergent]{
        \includegraphics[width=0.45\linewidth]{figures/angle-def/convergent-cond.pdf}
        \label{fig:supp:study:conditions:convergent}
    }%subfloat
    \Caption{
       Study conditions.
    }{
        All visualized conditions originate at a $+$ sign (near for divergent, far for convergent conditions), and target $\cdot$ signs.
        Leftward and rightward saccades are treated as equivalent in data analysis, but there are equal number of leftward and rightward conditions implemented.
    }
\label{fig:supp:study:conditions}
\end{figure}



==> paper-support.tex <==
\clearpage
\pagenumbering{roman}
\input{sec_supp}


==> tab_pilot_hmd.tex <==
\begin{table}[htb]
  \caption{Varjo Aero: relevant specifications.}
\begin{tabular}{c |c | c}
    \hline
    Resolution & Frequency & Peak Luminance \\
    \hline
     $2880 \times 2720$ & $90\ \text{Hz}$ & $150\ \text{cd}/\text{m}^2$\\
    \hline
    \hline
    Focal Distance & FoV & Supported IPD \\
    \hline
    $0.85\ \text{m}$ & $134^\circ$ (diagonal) & $59 - 71\ \text{mm}$\\
    \hline
    \hline
    Eye Tracker & Frequency & Accuracy\\
    \hline
    & $200\ \text{Hz}$ & $<1^\circ$\\
    \hline
\end{tabular}
\end{table}

